Weighted Emulators with Local Heaviest Edges Stretch for Undirected Graphs

We introduce a generalized family of $\left( 2\cdot \left\lfloor \frac{k}{2} \right\rfloor-1, 2\cdot \left\lceil \frac{k}{2} \right\rceil \cdot W_{1} +\max\left\{0,2\cdot\left(\left\lceil\frac{k}{2}\right\rceil-2\right)\right\}\cdot W_{2} \right)$-emulators with $\tilde O \left(n^{1+\frac{1}{k}}\right)$ edges, for any $k\in\mathbb{N}$, where $W_{i}$ is the $i$th heaviest edge on a shortest path between two vertices. Our construction generalizes the $+2W_{1}$-spanner of size $\tilde O\left(n^{\frac{3}{2}}\right)$ and the $+4W_{1}$-emulator of size $\tilde O \left(n^{\frac{4}{3}}\right)$, both by Elkin, Gitlitz and Neiman [DISC'21 and DICO'23]. When $k$ is even, these are $\left(k-1,k\cdot W_{1} + \left(k-4\right)\cdot W_{2}\right)$-emulators and when $k$ is odd, these are $\left(k-2,\left(k+1\right)\cdot W_{1} + \left(k-3\right) \cdot W_{2}\right)$-emulators. Our framework not only expands known constructions for weighted graphs but also yields an improved stretch over state of the art emulators and spanners for unweighted graphs within a specific distance regime. In particular, for all vertex pairs separated by a distance of $\delta \leq O\left(3^{k^{2}}\right)$, our construction improves upon the seminal additive $+\tilde O\left(\delta^{1-\frac{1}{k}}\right)$-emulator of size $\tilde O\left(n^{1+\frac{1}{2^{k+1}-1}}\right)$ by Thorup and Zwick [SODA'06].

==> Algorithms/APASP/+2Wi.tex <==
\begin{algorithm}[H]
\caption{$+2\sum_{i=1}^{k+1}{W_{i}}$-APASP$\left(G=\left(V,E,w\right)\right)$}\label{alg:+2Wi}

\textbf{Input:} An undirected non-negative weighted graph $G=\left(V,E,w\right)$ and $k\in \mathbb{N}$.

\textbf{Output:} A $+2\sum_{i=1}^{k+1}{W_{i}}$-APASP. 

\medskip

Let $\beta_{1},\ldots, \beta_{3k+2} \in \paren{ 0 , 1 }$ to be fixed later

Initialize $d$ as the edges' weights and $\infty$ otherwise

Set $S_0 \leftarrow V$

\For{$i \in \bracke{3k+2}$}
{
    Sample each vertex of $S_{i-1}$ with probability $n^{-\beta_i}$ to $S_{i}$
    
    For every  $u\in V$ find the pivot $p_{i}\paren{u}$ 

    Construct the edge set $D_{i}$

    Construct the edge set $E_{i}$ 
}

Set $S_{3k+3} \leftarrow \varnothing$

$D\leftarrow \mcup{D_{i}}{i=1}{k-1}$


\For{$i \in \pair{3k+2,\ldots,1,0}$}
{
    $Q_{i} \leftarrow \varnothing$

    \For{$j \in \bracce{0,1,\ldots,3k+2}$}
    {
        \For{$\ell \in \bracce{3k+1-i-j,3k+2-i-j,\ldots,3k+2}$}
        {
            $Q_{i} \leftarrow Q_{i} \cup \paren{S_{\ell}\times S_{j}}$
        }
    }

    \For{$s\in  S_{i}$}
    {
        Invoke SSSP from $s$ on $ G_{i} \paren{s} = \paren{ V,E_{i+1} \cup \paren{\bracce{s}\times V} \cup D \cup Q_{i} , d }$ and update $d$ accordingly
    }
}

\Return $d$

\end{algorithm}



==> Algorithms/Emulators/known/3ellplus4overellplus2.tex <==
\begin{algorithm}[H]
\caption{$\frac{3\ell+4}{\ell+2}$-APASP$\left(G=\left(V,E\right),w\right)$}\label{alg:3ellplus4overellplus2}
\textbf{Input:} An undirected graph $G=\left(V,E\right)$, a positive weight function $w:E\rightarrow\mathbb{R}^+$ and an integer $\ell\in\mathbb{N}$.

\textbf{Output:} A matrix $d$ which is a $\frac{3\ell+4}{\ell+2}$-APASP. 

\medskip

Let $\beta_{1},\ldots,\beta_{\ell+1} \in \paren{0,1}$ to be fixed later

Initialize $d$ as the edges' weights and $\infty$ otherwise

\For{$i \in \bracke{\ell}$}
{
    $\alpha_{i} \leftarrow \msum{\beta_{j}}{j=1}{i} $

    \For{$u\in V$}
    {
        Compute $\Gamma\paren{u,V,n^{\alpha_{i}}}$
    }

    Compute $S_{i}$ to be a hitting set to $\bracce{\Gamma\paren{u,V,n^{\alpha_{i}}} \mid u\in V}$

    Compute $\Gamma\paren{u,S_{i},n^{\beta_{i+1}}}$

    Compute the distances from any $u\in V$ to its pivot $p_{i}\paren{u}$ 

    Construct the set of edges $E_{S_{i}}$
}

\For{$\paren{x,y}\in E$}
{
    \For{$i \in \bracke{\ell+1}$}
    {
         \For{$v\in \Gamma\paren{y,S_{i-1},n^{\beta_{i}}}$}
        { 
            $d\bracke{p_{i}\paren{v},x}\leftarrow \mmin{d\bracke{p_{i}\paren{v},v}+d\bracke{v,y}+d\bracke{x,y}, d\bracke{p_{i}\paren{v},x}}$        
        }
    }
}

\For{$i \in \bracce{0}\cup \bracke{\ell+1}$}
{
    \For{$s\in  S_{i}$}
    {
        Invoke SSSP from $s$ on $G_{i} \paren{s} = \paren{ V,E_{ 
 S_{i+1}} \cup \paren{\bracce{s}\times V} \cup H \cup R_{i} , d }$ and update $d$ accordingly
    }
}

\For{$u,v\in V$}
{
    \For{$i \in \bracke{\ell+1}$}
    {
        \For{$s\in  \Gamma\paren{u,S_{i},n^{\beta_{i+1}}}$}
        {
            $d\bracke{u,v}\leftarrow \mmin{d\bracke{u,s}+d\bracke{s,v},d\bracke{u,v}}$
        }
    }
}

\For{$u,v\in V$} 
{           
  $\mmin{d\bracke{u,p_{i}\paren{u}}+d\bracke{p_{i}\paren{u},v},d\bracke{u,v}}{i=0}{\ell+1}$
}

\Return $d$
\end{algorithm}

==> Algorithms/Emulators/known/7over3.tex <==
\begin{algorithm}[H]
\caption{$\frac{7}{3}$-APASP$\left(G=\left(V,E\right),w\right)$}\label{alg:7over3}
\textbf{Input:} An undirected graph $G=\left(V,E\right)$ and a positive weight function $w:E\rightarrow\mathbb{R}^+$.

\textbf{Output:} A matrix $d$ which is a $\frac{7}{3}$-APASP. 

\medskip

Let $\beta,\gamma \in \paren{0,1}$ to be fixed later

Initialize $d$ as the edges' weights and $\infty$ otherwise

Compute $\Gamma\paren{u,V,n^{\beta}}$ (respectively, $\Gamma\paren{u,V,n^{\beta+\gamma}}$) for all $u\in V$

Compute $S_{1}$ (respectively, $S_{2}$) to be a hitting set to $\bracce{\Gamma\paren{u,V,n^{\beta}} \mid u\in V}$ (respectively, $\Gamma\paren{u,V,n^{\beta+\gamma}}$)

Compute the distances from any $u\in V$ to its pivot $p_{1}\paren{u}$ (respectively, $p_{2}\paren{u}$)

Construct the set of edges $E_{S_{1}}$ (respectively, $E_{S_{2}}$)

\For{$\paren{x,y}\in E$}
{
    \For{$v\in \Gamma\paren{y,V,n^{\beta}}$}
    {      
        \For{$i \in \bracce{0,1,2}$}
        {
            $d\bracke{p_{i}\paren{v},x}\leftarrow \mmin{d\bracke{p_{i}\paren{v},v}+d\bracke{v,y}+d\bracke{x,y}, d\bracke{p_{i}\paren{v},x}}$
        }
    }
}

\For{$i \in \bracce{0,1,2}$}
{
    \For{$s\in  S_{i}$}
    {
        Invoke SSSP from $s$ on $G_{i} \paren{s} = \left( V,E_{ 
 S_{i+1}} \cup \paren{\bracce{s}\times V} \cup H  , d \right)$ and update $d$ accordingly
    }
}

\For{$u,v\in V$}
{
    \For{$s\in  \Gamma\paren{u,S_{1},n^{\gamma}}$}
    {
        $d\bracke{u,v}\leftarrow \mmin{d\bracke{u,s}+d\bracke{s,v},d\bracke{u,v}}$
    }
}

\For{$u,v\in V$} 
{
    \For{$i \in \bracke{1,2}$}
    {
        $d\bracke{u,v}\leftarrow \mmin{d\bracke{u,p_{i}\paren{u}}+d\bracke{p_{i}\paren{u},v},d\bracke{u,v}}$
    }
}

\Return $d$
\end{algorithm}

==> Algorithms/Emulators/known/tz.tex <==
\begin{algorithm}[H]
\caption{ThorupZwick-Distance Oracle}\label{alg:tz}
\textbf{Input:} An undirected weighted graph $G=\left(V,E,w\right)$, vertices $u,v\in V$, hitting sets $S_{i}$ to $\Gamma\paren{u,V,n^{\beta_{1}+\ldots+\beta_{i}}}$, sets $\Gamma\paren{u,S_{i},n^{\beta_{i+1}}}\paren{x}$ for all $x\in V$ and $i\in \bracke{k}$, an integer $r\in\bracke{k}$ and a set of $\beta_1,\beta_2\ldots,\beta_{k+1}\in \paren{0,1}$.

\textbf{Output:} $d\bracke{u,v}$. 

\medskip

$i\leftarrow r$

\While{$p_{i}\paren{u}\notin \Gamma\paren{v,S_{i},n^{\beta_{i+1}}}$}
{
    $i\leftarrow i+1$

    Replace between $u,v$
}

\Return $d\bracke{u,p_{i}\paren{u}}+d\bracke{v,p_{i}\paren{v}}$
\end{algorithm}

==> Illustrations/Balls/ballexample.tex <==
\begin{figure}[H]
\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp6625860162276211] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.55 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (301.45,234.55) .. controls (272.97,209.21) and (270.06,166) .. (294.94,138.04) .. controls (319.82,110.09) and (363.07,107.97) .. (391.55,133.32) .. controls (420.03,158.67) and (422.94,201.87) .. (398.06,229.83) .. controls (373.18,257.78) and (329.93,259.9) .. (301.45,234.55) -- cycle ;
%Straight Lines [id:da9412047664314018] 
\draw    (314.73,189.53) -- (361.23,162.53) ;
%Straight Lines [id:da5938656329561427] 
\draw    (314.73,189.53) -- (358.73,226.2) ;
%Straight Lines [id:da15591646157325867] 
\draw    (358.73,226.2) -- (400.75,264) ;
%Straight Lines [id:da8588636129532099] 
\draw    (358.73,226.2) -- (434.75,226.5) ;
%Straight Lines [id:da3423424168072611] 
\draw    (400.75,264) -- (434.75,226.5) ;
%Straight Lines [id:da7252060609228765] 
\draw    (359.73,225.2) -- (434.25,164) ;
%Straight Lines [id:da8370853051570586] 
\draw    (434.25,164) -- (434.75,222.5) ;
%Straight Lines [id:da23613900566954826] 
\draw    (435.5,165.33) -- (471.75,201) ;
%Straight Lines [id:da18676055033971273] 
\draw    (438.25,162) -- (472.25,147) ;
%Straight Lines [id:da2707706875989797] 
\draw    (472.25,143) -- (472,110.67) ;
%Straight Lines [id:da8302620780031216] 
\draw    (364.23,160.53) -- (468.57,112.87) ;
%Straight Lines [id:da8037223017346966] 
\draw    (365.23,162.53) -- (434.25,163) ;
%Shape: Circle [id:dp40608497322126125] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (357.23,162.53) .. controls (357.23,160.32) and (359.02,158.53) .. (361.23,158.53) .. controls (363.44,158.53) and (365.23,160.32) .. (365.23,162.53) .. controls (365.23,164.74) and (363.44,166.53) .. (361.23,166.53) .. controls (359.02,166.53) and (357.23,164.74) .. (357.23,162.53) -- cycle ;
%Shape: Circle [id:dp26827319251987447] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354.73,226.2) .. controls (354.73,223.99) and (356.52,222.2) .. (358.73,222.2) .. controls (360.94,222.2) and (362.73,223.99) .. (362.73,226.2) .. controls (362.73,228.41) and (360.94,230.2) .. (358.73,230.2) .. controls (356.52,230.2) and (354.73,228.41) .. (354.73,226.2) -- cycle ;
%Straight Lines [id:da8476855593267647] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (500.25,180) -- (477.58,154.49) ;
\draw [shift={(476.25,153)}, rotate = 48.37] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp9709647852196648] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (310.73,189.53) .. controls (310.73,187.32) and (312.52,185.53) .. (314.73,185.53) .. controls (316.94,185.53) and (318.73,187.32) .. (318.73,189.53) .. controls (318.73,191.74) and (316.94,193.53) .. (314.73,193.53) .. controls (312.52,193.53) and (310.73,191.74) .. (310.73,189.53) -- cycle ;
%Shape: Circle [id:dp5706248374556] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.25,163) .. controls (430.25,160.79) and (432.04,159) .. (434.25,159) .. controls (436.46,159) and (438.25,160.79) .. (438.25,163) .. controls (438.25,165.21) and (436.46,167) .. (434.25,167) .. controls (432.04,167) and (430.25,165.21) .. (430.25,163) -- cycle ;
%Shape: Circle [id:dp6661137907917287] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468,110.67) .. controls (468,108.46) and (469.79,106.67) .. (472,106.67) .. controls (474.21,106.67) and (476,108.46) .. (476,110.67) .. controls (476,112.88) and (474.21,114.67) .. (472,114.67) .. controls (469.79,114.67) and (468,112.88) .. (468,110.67) -- cycle ;
%Shape: Circle [id:dp1158857638153572] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.25,147) .. controls (468.25,144.79) and (470.04,143) .. (472.25,143) .. controls (474.46,143) and (476.25,144.79) .. (476.25,147) .. controls (476.25,149.21) and (474.46,151) .. (472.25,151) .. controls (470.04,151) and (468.25,149.21) .. (468.25,147) -- cycle ;
%Shape: Circle [id:dp7673589811197465] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (467.75,201) .. controls (467.75,198.79) and (469.54,197) .. (471.75,197) .. controls (473.96,197) and (475.75,198.79) .. (475.75,201) .. controls (475.75,203.21) and (473.96,205) .. (471.75,205) .. controls (469.54,205) and (467.75,203.21) .. (467.75,201) -- cycle ;
%Shape: Circle [id:dp5265818224073935] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.75,226.5) .. controls (430.75,224.29) and (432.54,222.5) .. (434.75,222.5) .. controls (436.96,222.5) and (438.75,224.29) .. (438.75,226.5) .. controls (438.75,228.71) and (436.96,230.5) .. (434.75,230.5) .. controls (432.54,230.5) and (430.75,228.71) .. (430.75,226.5) -- cycle ;
%Shape: Circle [id:dp603509841517055] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (396.75,264) .. controls (396.75,261.79) and (398.54,260) .. (400.75,260) .. controls (402.96,260) and (404.75,261.79) .. (404.75,264) .. controls (404.75,266.21) and (402.96,268) .. (400.75,268) .. controls (398.54,268) and (396.75,266.21) .. (396.75,264) -- cycle ;

% Text Node
\draw (383.42,264.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (339.92,226.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (441.83,219.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (418,144) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (479.08,196.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (479.08,107.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{3}$};
% Text Node
\draw (479.25,142.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (357.25,169.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (394,213) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (473.83,121.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.5,163.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (373.33,246.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 2$};
% Text Node
\draw (327,207.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 2$};
% Text Node
\draw (397,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 3$};
% Text Node
\draw (328.5,163.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 3$};
% Text Node
\draw (424.33,191) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 9$};
% Text Node
\draw (452,156.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (446.5,185.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (412.17,121.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (416.83,244.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (507.57,185.27) node  [font=\tiny] [align=left] {\begin{minipage}[lt]{17.59pt}\setlength\topsep{0pt}
\textcolor[rgb]{0.29,0.56,0.89}{$\displaystyle p_{S}( u)$}
\end{minipage}};
% Text Node
\draw (295.75,190.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (307.47,127.01) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 45; green, 127; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle ball( u,A,S)$};


\end{tikzpicture}




\caption{\label{fig:ballexample} The ball $ball \left(u,A,S\right)$, where $A=\left\{ a_1,a_2,a_3\right\}$ and $S=\left\{s_1,s_2,s_3\right\}$. The pivot for $u$ is $p\left(u\right) = s_2$ with $\delta\left(u,S\right) = 5$.}
\end{figure}\vspace{-4mm}

==> Illustrations/Balls/inneredgesexample.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da87840787155437] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (315.01,190.03) -- (361.51,163.03) ;
%Straight Lines [id:da052344792013143016] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (315.01,190.03) -- (359.01,226.7) ;
%Straight Lines [id:da704512876406874] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (359.01,226.7) -- (401.03,264.5) ;
%Straight Lines [id:da2529965611042688] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (359.01,226.7) -- (435.03,227) ;
%Straight Lines [id:da038558601052662844] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (401.03,264.5) -- (435.03,227) ;
%Straight Lines [id:da1453158167020543] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (360.01,225.7) -- (434.53,164.5) ;
%Straight Lines [id:da8496894787108054] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (434.53,164.5) -- (435.03,223) ;
%Straight Lines [id:da15583751877941343] 
\draw    (435.78,165.83) -- (472.03,201.5) ;
%Straight Lines [id:da6954206584025682] 
\draw    (438.53,162.5) -- (472.53,147.5) ;
%Straight Lines [id:da9064565291303313] 
\draw    (472.53,143.5) -- (472.28,111.17) ;
%Straight Lines [id:da53256747981667] 
\draw    (364.51,161.03) -- (468.85,113.37) ;
%Straight Lines [id:da35419788722237744] 
\draw [color={rgb, 255:red, 13; green, 113; blue, 228 }  ,draw opacity=1 ]   (365.51,163.03) -- (434.53,163.5) ;
%Shape: Circle [id:dp31720811305789964] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (357.51,163.03) .. controls (357.51,160.82) and (359.3,159.03) .. (361.51,159.03) .. controls (363.72,159.03) and (365.51,160.82) .. (365.51,163.03) .. controls (365.51,165.24) and (363.72,167.03) .. (361.51,167.03) .. controls (359.3,167.03) and (357.51,165.24) .. (357.51,163.03) -- cycle ;
%Shape: Circle [id:dp5265937509664673] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (355.01,226.7) .. controls (355.01,224.49) and (356.8,222.7) .. (359.01,222.7) .. controls (361.22,222.7) and (363.01,224.49) .. (363.01,226.7) .. controls (363.01,228.91) and (361.22,230.7) .. (359.01,230.7) .. controls (356.8,230.7) and (355.01,228.91) .. (355.01,226.7) -- cycle ;
%Shape: Circle [id:dp24609937249348568] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (311.01,190.03) .. controls (311.01,187.82) and (312.8,186.03) .. (315.01,186.03) .. controls (317.22,186.03) and (319.01,187.82) .. (319.01,190.03) .. controls (319.01,192.24) and (317.22,194.03) .. (315.01,194.03) .. controls (312.8,194.03) and (311.01,192.24) .. (311.01,190.03) -- cycle ;
%Shape: Circle [id:dp9874523059430802] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.53,163.5) .. controls (430.53,161.29) and (432.32,159.5) .. (434.53,159.5) .. controls (436.74,159.5) and (438.53,161.29) .. (438.53,163.5) .. controls (438.53,165.71) and (436.74,167.5) .. (434.53,167.5) .. controls (432.32,167.5) and (430.53,165.71) .. (430.53,163.5) -- cycle ;
%Shape: Circle [id:dp8586237542464736] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.28,111.17) .. controls (468.28,108.96) and (470.07,107.17) .. (472.28,107.17) .. controls (474.49,107.17) and (476.28,108.96) .. (476.28,111.17) .. controls (476.28,113.38) and (474.49,115.17) .. (472.28,115.17) .. controls (470.07,115.17) and (468.28,113.38) .. (468.28,111.17) -- cycle ;
%Shape: Circle [id:dp8552923192966435] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.53,147.5) .. controls (468.53,145.29) and (470.32,143.5) .. (472.53,143.5) .. controls (474.74,143.5) and (476.53,145.29) .. (476.53,147.5) .. controls (476.53,149.71) and (474.74,151.5) .. (472.53,151.5) .. controls (470.32,151.5) and (468.53,149.71) .. (468.53,147.5) -- cycle ;
%Shape: Circle [id:dp6801603655991799] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ] (468.03,201.5) .. controls (468.03,199.29) and (469.82,197.5) .. (472.03,197.5) .. controls (474.24,197.5) and (476.03,199.29) .. (476.03,201.5) .. controls (476.03,203.71) and (474.24,205.5) .. (472.03,205.5) .. controls (469.82,205.5) and (468.03,203.71) .. (468.03,201.5) -- cycle ;
%Shape: Circle [id:dp7631537577629186] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (431.03,227) .. controls (431.03,224.79) and (432.82,223) .. (435.03,223) .. controls (437.24,223) and (439.03,224.79) .. (439.03,227) .. controls (439.03,229.21) and (437.24,231) .. (435.03,231) .. controls (432.82,231) and (431.03,229.21) .. (431.03,227) -- cycle ;
%Shape: Circle [id:dp4241349705641584] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (397.03,264.5) .. controls (397.03,262.29) and (398.82,260.5) .. (401.03,260.5) .. controls (403.24,260.5) and (405.03,262.29) .. (405.03,264.5) .. controls (405.03,266.71) and (403.24,268.5) .. (401.03,268.5) .. controls (398.82,268.5) and (397.03,266.71) .. (397.03,264.5) -- cycle ;

% Text Node
\draw (383.7,265) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (340.2,227) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (442.11,219.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (418.28,144.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (479.36,197) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (479.36,107.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{3}$};
% Text Node
\draw (479.53,142.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (357.53,170) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (394.28,213.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 1$};
% Text Node
\draw (474.11,121.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.78,164) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 1$};
% Text Node
\draw (373.61,246.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 2$};
% Text Node
\draw (327.28,207.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 2$};
% Text Node
\draw (397.28,193.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 3$};
% Text Node
\draw (328.78,164.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 3$};
% Text Node
\draw (424.61,191.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 9$};
% Text Node
\draw (452.28,156.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 4$};
% Text Node
\draw (446.78,185.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (412.45,122.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (417.11,245) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle 4$};
% Text Node
\draw (296.03,190.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};


\end{tikzpicture}

\caption{\label{fig:inneredgesexample} The inner-edges $E_{S}$ of all vertices $V$, in relation to $S$.}
\end{figure}

==> Illustrations/Balls/nearestexample.tex <==
\begin{figure}[H]
\centering

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp6625860162276211] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.55 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (301.45,234.55) .. controls (272.97,209.21) and (270.06,166) .. (294.94,138.04) .. controls (319.82,110.09) and (363.07,107.97) .. (391.55,133.32) .. controls (420.03,158.67) and (422.94,201.87) .. (398.06,229.83) .. controls (373.18,257.78) and (329.93,259.9) .. (301.45,234.55) -- cycle ;
%Straight Lines [id:da9412047664314018] 
\draw    (314.73,189.53) -- (361.23,162.53) ;
%Straight Lines [id:da5938656329561427] 
\draw    (314.73,189.53) -- (358.73,226.2) ;
%Straight Lines [id:da8588636129532099] 
\draw    (358.73,226.2) -- (434.75,226.5) ;
%Straight Lines [id:da7252060609228765] 
\draw    (359.73,225.2) -- (434.25,164) ;
%Straight Lines [id:da8370853051570586] 
\draw    (434.25,164) -- (434.75,222.5) ;
%Straight Lines [id:da23613900566954826] 
\draw    (198.43,200.43) -- (248.43,190.43) ;
%Straight Lines [id:da18676055033971273] 
\draw    (198.43,200.43) -- (255,153.67) ;
%Straight Lines [id:da2707706875989797] 
\draw    (252.43,186.43) -- (259,153.67) ;
%Straight Lines [id:da8302620780031216] 
\draw    (263.43,153.43) -- (357.23,162.53) ;
%Straight Lines [id:da8037223017346966] 
\draw    (365.23,162.53) -- (434.25,163) ;
%Shape: Circle [id:dp40608497322126125] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (357.23,162.53) .. controls (357.23,160.32) and (359.02,158.53) .. (361.23,158.53) .. controls (363.44,158.53) and (365.23,160.32) .. (365.23,162.53) .. controls (365.23,164.74) and (363.44,166.53) .. (361.23,166.53) .. controls (359.02,166.53) and (357.23,164.74) .. (357.23,162.53) -- cycle ;
%Shape: Circle [id:dp26827319251987447] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354.73,226.2) .. controls (354.73,223.99) and (356.52,222.2) .. (358.73,222.2) .. controls (360.94,222.2) and (362.73,223.99) .. (362.73,226.2) .. controls (362.73,228.41) and (360.94,230.2) .. (358.73,230.2) .. controls (356.52,230.2) and (354.73,228.41) .. (354.73,226.2) -- cycle ;
%Shape: Circle [id:dp9709647852196648] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (310.73,189.53) .. controls (310.73,187.32) and (312.52,185.53) .. (314.73,185.53) .. controls (316.94,185.53) and (318.73,187.32) .. (318.73,189.53) .. controls (318.73,191.74) and (316.94,193.53) .. (314.73,193.53) .. controls (312.52,193.53) and (310.73,191.74) .. (310.73,189.53) -- cycle ;
%Shape: Circle [id:dp5706248374556] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.25,163) .. controls (430.25,160.79) and (432.04,159) .. (434.25,159) .. controls (436.46,159) and (438.25,160.79) .. (438.25,163) .. controls (438.25,165.21) and (436.46,167) .. (434.25,167) .. controls (432.04,167) and (430.25,165.21) .. (430.25,163) -- cycle ;
%Shape: Circle [id:dp6661137907917287] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (255,153.67) .. controls (255,151.46) and (256.79,149.67) .. (259,149.67) .. controls (261.21,149.67) and (263,151.46) .. (263,153.67) .. controls (263,155.88) and (261.21,157.67) .. (259,157.67) .. controls (256.79,157.67) and (255,155.88) .. (255,153.67) -- cycle ;
%Shape: Circle [id:dp1158857638153572] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (248.43,190.43) .. controls (248.43,188.22) and (250.22,186.43) .. (252.43,186.43) .. controls (254.64,186.43) and (256.43,188.22) .. (256.43,190.43) .. controls (256.43,192.64) and (254.64,194.43) .. (252.43,194.43) .. controls (250.22,194.43) and (248.43,192.64) .. (248.43,190.43) -- cycle ;
%Shape: Circle [id:dp7673589811197465] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (194.43,200.43) .. controls (194.43,198.22) and (196.22,196.43) .. (198.43,196.43) .. controls (200.64,196.43) and (202.43,198.22) .. (202.43,200.43) .. controls (202.43,202.64) and (200.64,204.43) .. (198.43,204.43) .. controls (196.22,204.43) and (194.43,202.64) .. (194.43,200.43) -- cycle ;
%Shape: Circle [id:dp5265818224073935] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (430.75,226.5) .. controls (430.75,224.29) and (432.54,222.5) .. (434.75,222.5) .. controls (436.96,222.5) and (438.75,224.29) .. (438.75,226.5) .. controls (438.75,228.71) and (436.96,230.5) .. (434.75,230.5) .. controls (432.54,230.5) and (430.75,228.71) .. (430.75,226.5) -- cycle ;
%Straight Lines [id:da295580442805107] 
\draw    (248.43,190.43) -- (314.73,189.53) ;

% Text Node
\draw (339.92,226.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (443.83,219.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{2}$};
% Text Node
\draw (443,155) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (192.08,205.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle a_{3}$};
% Text Node
\draw (254.08,132.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle b_{3}$};
% Text Node
\draw (247.51,196.43) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle b_{4}$};
% Text Node
\draw (357.25,169.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,xslant=-0.03] [align=left] {$\displaystyle u$};
% Text Node
\draw (397,213) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (275.83,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (389.5,163.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (327,207.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (398,193.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (328.5,163.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (424.33,191) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 9$};
% Text Node
\draw (221,159.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 5$};
% Text Node
\draw (223.17,198.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 6$};
% Text Node
\draw (295.75,190.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xslant=-0.03] [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (307.47,127.01) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 45; green, 127; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \Gamma ( u,A,2)$};
% Text Node
\draw (295.94,142.04) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};
% Text Node
\draw (260.17,165.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle 1$};


\end{tikzpicture}






\caption{\label{fig:nearestexample} The set $\Gamma \paren{u,A,2}$, where $A=\left\{ a_1,a_2,a_3\right\}$.}
\end{figure}\vspace{-2mm}
